An Assessment Methodology and Instrument for Cybersecurity: The Ireland Use Case

Governments around the world are required to strengthen their national cybersecurity capabilities to respond effectively to the growing, changing, and sophisticated cyber threats and attacks, thus protecting society and the way of life as a whole. Responsible government institutions need to revise, evaluate, and bolster their national cybersecurity capabilities to fulfill the new requirements, for example regarding new trends affecting cybersecurity, key supporting laws and regulations, and implementations risk and challenges. This report presents a comprehensive assessment instrument for cybersecurity at the national level in order to help countries to ensure optimum response capability and more effective use of critical resources of each state. More precisely, the report - builds a common understanding of the critical cybersecurity capabilities and competence to be assessed at the national level, - adds value to national strategic planning and implementation which impact the development and adaptation of national cybersecurity strategies, - provides an overview of the assessment approaches at the national level, including capabilities, frameworks, and controls, - introduces a comprehensive cybersecurity instrument for countries to determine areas of improvement and develop enduring national capabilities, - describes how to apply the proposed national cybersecurity assessment framework in a real-world case, and - presents the results and lessons learned of the application of the assessment framework at the national level to assist governments in further building cybersecurity capabilities.

==> drafts.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
\multirow{2}{*}{No} & \multirow{2}{*}{Qualitative Findings -   Questions}                                                                                                                                                           & \multirow{2}{*}{Ireland Evidence}                                      & \multirow{2}{*}{Ireland Findings}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\
                    &                                                                                                                                                                                                               &                                                                        &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\multirow{2}{*}{1}  & \multirow{2}{*}{What is the government cybersecurity policy unit?}                                                                                                                                            & The Department of the   Environment, Climate and Communications (DECC) & The   DECC creates policies for Communications and Digital including Cybersecurity                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & The National Cyber Security Centre (NSCS)                              & The   NCSC of Ireland  provides enhanced   services to government agencies and critical infrastructure providers to   assist them in defending against cyber security incidents, current threats   and vulnerabilities associated with network information security. The NCSC   team works alongside government agencies and private industry to facilitate   secure systems and information. NCSC participates in national, EU and   international emergency response exercises and provides expert advice to   government departments and industry on specific cyber threats and incidents.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
2                   & What   are the government committees, working groups, etc. for cybersecurity?                                                                                                                                 & Data Protection   Commission (DPC)                                     & The   DPC is the national independent authority responsible for upholding the   fundamental right of individuals in the EU to have their personal data   protected. The DPC is the Irish supervisory authority for the General Data   Protection Regulation (GDPR), and also has functions and powers related to   other important regulatory frameworks including the Irish ePrivacy   Regulations (2011) and the EU Directive known as the Law Enforcement   Directive.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\multirow{2}{*}{3}  & \multirow{2}{*}{What is the government national-level   cybersecurity strategy or other equivalent document?}                                                                                                 & \multirow{2}{*}{National   CS Strategy}                                & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}The   National Cyber Security Strategy (December 2019) follows on from the   country's first strategy. It is a broader and more comprehensive document   than the last one, and is informed by the operational experience gained by   the National Cyber Security Centre (NCSC) from 2015 to 2019, and from ongoing   national and international engagements in the area.\\      \\      The vision behind the 2019 Strategy is for Ireland to continue to safely   enjoy the benefits of the digital revolution and to play a full part in   shaping the future of the Internet. This vision will be achieved   through:\\      - the protection of the State, its people, and its critical national   infrastructure from cyber threats\\      - the development of the capacity of the State, of research institutions,   of businesses and of the people, to both better understand and manage the   nature of the challenges we face\\      - the engagement by the State, nationally and internationally, in a   strategic manner, supporting a free, open, peaceful and secure cyber space\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\
                    &                                                                                                                                                                                                               &                                                                        &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\multirow{5}{*}{4}  & \multirow{5}{*}{What is the government implementation plan to   the national-level cybersecurity strategy or other equivalent document?}                                                                      & National CS   Strategy                                                 & Appendix   1 contains the list of actions for implementing the cybersecurity   strategy                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & Operators of Essential Service                                         & The   NIS Compliance Guidelines for Operators of Essential Service (OES)   establishes a set of Guidelines designed to assist OES in meeting their   network and information system security and incident reporting requirements   under Regulations 17 and 18 of the NIS Regulations. As part of the EU   Cybersecurity strategy the European Commission, the EU Network and   Information Security (NIS) Directive (see EU 2016/1148) is the first piece of   EU-wide cybersecurity legislation. The goal is to enhance cybersecurity across   the EU.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & Digital Service Providers                                              & The   Information Note for Digital Service Providers assists Digital Service   Providers in understanding their obligations in relation to compliance with   the NIS Directive. As part of the EU Cybersecurity strategy the European   Commission, the EU Network and Information Security (NIS) Directive (see EU   2016/1148) is the first piece of EU-wide cybersecurity legislation. The goal   is to enhance cybersecurity across the EU.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & IS Management                                                          & The   Advice Note: Considering Information Security Management Supporting the   Public Service ICT Strategy contains the suggested strategies and activities   to enhance information security. t aims to assist Public Bodies in making   informed, risk-based decisions in relation to the improvement of Information   Security within their organisation.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & CS Guidance for Business                                               & The   12 Steps to Cyber Security Guidance on Cyber Security for Irish Business is   intended to be used by businesses as a suggested activity plan which may be   undertaken on a month-by-month basis over a suggested 12 month period to   improve cyber resilience.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
5                   & What   is the government entity unit that is specialised in national strategic cyber   threats?                                                                                                               & The National   Cyber Security Centre (NSCS)                            & The NCSC of Ireland  provides enhanced services to government   agencies and critical infrastructure providers to assist them in defending   against cyber security incidents, current threats and vulnerabilities   associated with network information security. The NCSC team works alongside   government agencies and private industry to facilitate secure systems and   information. NCSC participates in national, EU and international emergency   response exercises and provides expert advice to government departments and   industry on specific cyber threats and incidents.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multirow{3}{*}{6}  & \multirow{3}{*}{What are the cyber threat reports published by   the government?}                                                                                                                             & \multirow{2}{*}{The National Cyber Security   Centre (NSCS)}           & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}The   National Cyber Security Centre (NCSC) is regularly publishing Alerts \&   Advisories on cyber security issues that may affect Ireland   (https://www.ncsc.gov.ie/news/) The latest published alerts are the   following: \\      - 11-03-2021 Critical Vulnerabilities in F5 products\\      - 10-03-2021 Critical Vulnerabilities in Microsoft Exchange Servers Update   2 \\      - 25-02-2021 Unauthorised RCE in VMware vCenter \& ESXi \\      - 10-02-2021 Windows TCP/IP Remote Code Execution \& DoS Vulnerabilities\\      - 25-01-2021 SonicWall Vulnerability\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\
                    &                                                                                                                                                                                                               &                                                                        &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & The European   Union Agency for Cybersecurity (ENISA)                  & \begin{tabular}[c]{@{}l@{}}ENISA   is the Union’s agency dedicated to achieving a high common level of   cybersecurity across Europe. ENISA provides the reports EU on threats as   below:\\      - ENISA (Annual) Threat Landscape (ETL) Report provides an overview of   threats, together with current and emerging trends. For example, ENISA Threat   Landscape 2020 - List of top 15 threats.\\      \\      - ENISA Advisory Info Notes provides the information in relation to the   latest threats and vulnerabilities.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\multirow{4}{*}{7}  & \multirow{4}{*}{What are the government cyber safety and   security websites?}                                                                                                                       & The Department   of the Environment, Climate and Communications (DECC) & It   creates policies for Communications and Digital including Cybersecurity   (https://www.gov.ie/en/policy-information/5e101b-network-and-information-security-cyber-security/)                                                                                                           \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & The National   Cyber Security Centre (NSCS)                            & It   is  the primary Cyber Security   authority in the State. The NCSC of Ireland    provides enhanced services to government agencies and critical   infrastructure providers to assist them in defending against cyber security   incidents, current threats and vulnerabilities associated with network   information security (https://www.ncsc.gov.ie/)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & CSIRT-IE                                                               & It   is responsible of the incident response for national cyber security incidents   at the government and national levels (https://www.ncsc.gov.ie/CSIRT/)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & Data Protection Commission (DPC)                                       & It   is is the national independent authority responsible for upholding the   fundamental right of individuals in the EU to have their personal data   protected. The DPC is the Irish supervisory authority for the General Data   Protection Regulation (GDPR). https://www.dataprotection.ie)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multirow{2}{*}{8}  & \multirow{2}{*}{What is the training on cibersecurity offered by   government?}                                                                                                                               & National CS   Strategy                                                 & \begin{tabular}[c]{@{}l@{}}One   of the main objectives of the National Cybersecurity Strategy is to invest in   educational initiatives to prepare the workforce for advanced IT and   cybersecurity careers.  These are the   main cybersecurity programs at the national level:\\      \\      Bachelor’s level cyber security programmes: \\        -https://www.wit.ie/courses/bsc\_hons\_in\_computer\_forensics\_and\_security\\      -   https://www.itcarlow.ie/courses/type/undergraduate-cao-courses/computing-networking-courses/bsc-science-cybercrime-itsecurity-cw227.htm   \\      -   https://www.tudublin.ie/study/undergraduate/courses/computing-dig-forensics-and-cyber-sec-tu863/\\       Master’s level cyber security   programmes: \\      - http://www.itb.ie/StudyatITB/bn528.html \\      - http://www.ucd.ie/cci/education/prospective\_students/msc\_difc.html   https://www.griffith.ie/faculties/computing/courses/master-science-network-and-info\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & ISACA Cybersecurity Professional Association                           & ISACA   is an international professional association focused on IT (information   technology) governance. It offers training and certification programs and it   is the creator of the COBIT framework. The ISACA Ireland Chapter's aim is to   sponsor local educational seminars and workshops, conduct regular chapter   meetings, and help to further promote and elevate the visibility of the IS   audit, control and security profession throughout the island of   Ireland.(http://www.isaca.org/chapters5/ireland/)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
9                   & What   are the international cooperation activites of government dedicated to cyber   security  (e.g. FIRST)?                                                                                                 & CSIRT-IE                                                               & The CSIRT-IE is   member of FIRST. FIRST's objective is to bring together incident response and   security teams from every country across the world to ensure a safe internet   for all.(https://www.first.org/members/teams/csirt-ie)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
10                  & What   are the government cybersecurity guidelines/notes for the digital service   providers?                                                                                                                 & Digital Service   Providers                                            & The   Information Note for Digital Service Providers assists Digital Service   Providers (i.e., Online marketplaces, Online search engines, and Cloud   computing services) in understanding their obligations in relation to   compliance with the NIS Directive.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
11                  & What   are the government cybersecurity guidelines/notes for operators of essential   services?                                                                                                               & Operators of Essential Service                                         & The NIS Compliance Guidelines   for Operators of Essential Service (OES)    (including digital infrastructure) establishes a set of Guidelines   designed to assist OES in meeting their network and information system security   and incident reporting requirements under Regulations 17 and 18 of the NIS   Regulations                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multirow{2}{*}{12} & \multirow{2}{*}{What evidence of the effective implementation of   cyber/information security policies (e.g. audit result, documentation,   specific report) is provided by operators of essential services?} & \multirow{2}{*}{Security Regulation and Law}                           & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}S.I. No. 360/2018 - European Union (Measures for   a High Common Level of Security of Network and Information Systems)   Regulations 2018\\      IMPLEMENTATION AND ENFORCEMENT\\      Security assessment\\      27. (1)(a) The competent authority referred to in Regulation 7(1) may, in   relation to those sectors in respect of which it is designated as the   competent authority, carry out an assessment, whether by means of a security   audit or otherwise, of the compliance by an operator of essential services   with its obligations under Regulations 17 and 18 and for that purpose may   appoint an independent person or auditor to carry out the assessment on its   behalf.\\      (b) The competent authority referred to in Regulation 8 may, in relation to   a relevant digital service provider, carry out an assessment, whether by   means of a security audit or otherwise, of the compliance by a relevant   digital service provider with its obligations under Regulations 21 and 22 and   for that purpose may appoint an independent person or auditor to carry out   the assessment on its behalf.\\      (2) A competent authority referred to in paragraph (1) may request an   operator of essential services or a relevant digital service provider, as the   case may be, to provide the competent authority with—\\      (a) the information necessary for that competent authority to assess the   security of the network and information systems of the operator or provider,   as the case may be, including documented security policies, and\\      (b) evidence of the effective implementation by the operator or provider,   as the case may be, of security policies including the implementation of any   recommendations made on foot of a security audit or other assessment.\end{tabular}} \\
                    &                                                                                                                                                                                                               &                                                                        &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
13                  & What   are the government legal acts for personal data protection?                                                                                                                                            & Data Protection   Regulation                                           & \begin{tabular}[c]{@{}l@{}}From 25 May 2018   the key legislative frameworks are:\\      - General Data Protection Regulation (GDPR)\\      - Data Protection Act 2018\\      - the “Law Enforcement Directive” (Directive (EU) 2016/680) which has been   transposed into Irish law by way of the Data Protection Act 2018\\      - the Data Protection Acts 1988 and 2003\\      - the 2011 “ePrivacy Regulations” (S.I. No. 336 of 2011 – the European   Communities (Electronic Communications Networks and Services) (Privacy And   Electronic Communications) Regulations 2011)\\        (https://www.dataprotection.ie/en/dpc-guidance/law/data-protection-legislation)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multirow{2}{*}{14} & \multirow{2}{*}{What are the government units (CSIRT, CERT, CIRT, etc.)   specialised in national-level cyber incident detection and response?}                                                               & \multirow{2}{*}{CSIRT-IE}                                              & \multirow{2}{*}{The government has a unit (CSIRT, CERT, CIRT,   etc.) that is specialised in national-level cyber incident detection and   response. The CSIRT-IE is responsible of the incident response for national   cyber security incidents at the government and national levels.}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\
                    &                                                                                                                                                                                                               &                                                                        &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\multirow{3}{*}{15} & \multirow{3}{*}{What are the government authorities that digital   service providers and operators of essential services must notify of   cybersecurity incidents?}                                           & OES Incident   Notification Form                                       & Operators   of Essential Services (OES) are required to report incidents which fall under   the scope of the NIS Directive. A reportable incident is any incident which   has a significant impact on the continuity of an essential service which an   Operator of Essential Services provides. OES have to notify the CSIRT of an   incident by using the "Operators of Essential Services: Incident   Notification Form"                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & \multirow{2}{*}{Incident Report Form}                                  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}As stated in Article 16 (4) of the NIS   Directive, in order to determine whether the impact of an incident is   substantial, the following parameters in particular shall be taken into   account:\\      - The number of users affected by the incident, in particular users relying   on the service for the provision of their own services;\\      - The duration of the incident;\\      - The geographical spread with regard to the area affected by the   incident;\\      - The extent of the disruption of the functioning of the service;\\      - The extent of the impact on economic and societal activities.\\      \\      Digital service providers have to notify the CSIRT of an incident by by   using the "Digital Service Providers: Incident Notification Form"\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\
                    &                                                                                                                                                                                                               &                                                                        &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\multirow{4}{*}{16} & \multirow{4}{*}{What is the government crisis management plan   for large-scale cyber incidents?}                                                                                                             & Operators   of Essential Service                                       & Appendix B:   Security Guidelines Category: Service Protection Policies, Processes and   Procedures (PR.SP) Subcategory PR.SP-9: Response plans (Incident Response and   Business Continuity) and recovery plans (Incident Recovery and Disaster   Recovery) are in place and managed Subcategory PR.SP-10: Response and   recovery plans are tested                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & Digital Service Providers                                              & Section 3.1:   Article 16 (1) Business continuity management referred to in point (c) of   Article 16(1) of Directive (EU)2016/1148 means the capability of an   organisation to maintain or as appropriate restorethe delivery of services at   acceptable predefined levels following a disruptive incident andshall   include: (a)the establishment and the use of contingency plans based on a   business impactanalysis for ensuring the continuity of the services provided   by digital service providerswhich shall be assessed and tested on a regular   basis for example, through exercises; (b)disaster recovery capabilities which   shall be assessed and tested on a regular basisfor example, through   exercises.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & IS Management                                                          & Appendix   C: Information Security Frameworks ISO 27002 (A.17) ENISA (D6)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & CS Guidance for Business                                               & STEP   9. Adopt a risk-based approach to resilience                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
\multirow{2}{*}{17} & \multirow{2}{*}{What are the cybersecurity standards referenced   by the government?}                                                                                                                         & Operators of   Essential Service                                       & \begin{tabular}[c]{@{}l@{}}Appendix B:   Security Guidelines\\      · CIS CSC\\      · COBIT 5\\      · ISA 62443-2-1:2009\\      · ISA 62443-3-3:2013\\      · ISO/IEC 27001:2013\\      · NIST SP 800-53 Rev. 4\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & IS Management                                                          & \begin{tabular}[c]{@{}l@{}}Appendix   C: Information Security Frameworks\\      1. ISO/IEC 27001 and ISO/IEC 27K Series \\      2. ENISA – Technical Guideline on Security Measures\\      3. National Institute of Standards and Technology (NIST)\\      4. NIST Risk Management Framework (RMF)\\      5. NIST Cybersecurity Framework\\      6. ISACA COBIT 5 for Information Security\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multirow{5}{*}{18} & \multirow{5}{*}{Is there any specific cybersecurity information   for emerging technologies (AI, ML, etc.), cloud services, and operational   technologies (OT) (e.g., asset management, OT devices)?}        & National CS   Strategy                                                 & Executive   Summary (some emerging technologies listed)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & AI Cybersecurity   Challenges                                          & This report   presents the Agency’s active mapping of the AI cybersecurity ecosystem and   its Threat Landscape, realised with the support of the Ad-Hoc Working Group   on Artificial Intelligence Cybersecurity.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & IS Management                                                          & Section: Other   Useful Sources                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & CS Guidance for Business                                               & Section:   Background (IoT mentioned)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \cline{3-4} 
                    &                                                                                                                                                                                                               & AmCham GCS Report                                                      & The main trends in the 2018   cyberthreat landscape, as identified by the European Union Agency for Network   and Information Security (ENISA) 19 showcase a range of hot-button issues                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\end{tabular}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{No.} & \multirow{2}{*}{Question}                                                                                                                              & \multirow{2}{*}{Evidence}                             & \multirow{2}{*}{Findings}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & \multirow{2}{*}{Maturity Level} \\
                     &                                                                                                                                                        &                                                       &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            &                                 \\ \hline
\multirow{4}{*}{1}   & \multirow{4}{*}{To what extent are   policies, laws, and guidelines for information security related to VTI\&CM   established?}                        & National CS   Strategy                                & \begin{tabular}[c]{@{}l@{}}The vision   behind the 2019 Strategy is for Ireland to continue to safely enjoy the   benefits of the digital revolution and to play a full part in shaping the   future of the Internet. This vision will be achieved through:\\      - the protection of the State, its people, and its critical national   infrastructure from cyber threats\\      - the development of the capacity of the State, of research institutions,   of businesses and of the people, to both better understand and manage the   nature of the challenges we face\\      - the engagement by the State, nationally and internationally, in a   strategic manner, supporting a free, open, peaceful and secure cyber space\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                           & \multirow{4}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & The   NIS Compliance Guidelines for Operators of Essential Service (OES)   establishes a set of Guidelines designed to assist OES in meeting their   network and information system security and incident reporting requirements   under Regulations 17 and 18 of the NIS Regulations                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Digital Service Providers                             & The   Information Note for Digital Service Providers assists Digital Service   Providers in understanding their obligations in relation to compliance with   the NIS Directive                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & Ireland   has developed guidelines for businesses to develop/adopt policies and   standards (security policy, data protection policy, malware protection   policy, remote access policy, etc.), as well as a programme to  monitor/measure compliance.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &                                 \\ \hline
\multirow{5}{*}{2}   & \multirow{5}{*}{To   what extent are there guidelines and regulations for development and   execution of information security strategies established?} & National   CS Strategy                                & \begin{tabular}[c]{@{}l@{}}The   Appendix 1 of the National Cybersecurity Strategy \\       contains the list of actions for   implementing the sybersecurity strategy\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & \multirow{5}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & The   NIS Compliance Guidelines for Operators of Essential Service (OES)   establishes a set of Guidelines designed to assist OES in meeting their   network and information system security and incident reporting requirements   under Regulations 17 and 18 of the NIS Regulations                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Digital Service Providers                             & The   Information Note for Digital Service Providers assists Digital Service   Providers in understanding their obligations in relation to compliance with   the NIS Directive                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & \begin{tabular}[c]{@{}l@{}}The   Advice Note: Considering Information Security Management\\      Supporting the Public Service ICT Strategy contains the suggested   strategies and activities to enhance information security\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & \begin{tabular}[c]{@{}l@{}}The   12 Steps to Cyber Security Guidance on Cyber Security for Irish Business is   intended to be used by businesses as  a   suggested activity plan which may be undertaken on\\      a month-by-month basis over a suggested 12 month period to improve cyber   resilience\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                 \\ \hline
\multirow{2}{*}{3}   & \multirow{2}{*}{To   what extent are governance structures for    information security related to VTI\&CM established?}                                & National   CS Strategy                                & The National Cyber Security Centre (NCSC)   will remain the primary Cyber Security authority in the State. The NCSC of   Ireland  provides enhanced services to   government agencies and critical infrastructure providers to assist them in   defending against cyber security incidents, current threats and   vulnerabilities associated with network information security. The NCSC team   works alongside government agencies and private industry to facilitate secure   systems and information. NCSC participates in national, EU and international   emergency response exercises and provides expert advice to government   departments and industry on specific cyber threats and incidents                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \multirow{2}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & Requirements for CSIRTs                               & The   government has a unit (CSIRT, CERT, CIRT, etc.) that is specialised in   national-level cyber incident detection and response. The CSIRT-IE is   responsible of the incident response for national cyber security incidents at   the government and national levels.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 &                                 \\ \hline
\multirow{4}{*}{4}   & \multirow{4}{*}{To what extent are responsibilities, penalties,   incentive models, and audit options established?}                                    & National   CS Strategy                                & The   NCSC has developed significantly in terms of capacity and resources, and its   roles have been formally established in law, including responsibilities   around Critical National Infrastructure protection and dealing with EU   requirements around the security of some. This document also focuses on the   ongoing compliance and audit programmes to mitigate risks to key services.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & \multirow{4}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & Requirements for CSIRTs                               & The   status of CSIRT-IE and its roles and functions are defined and documented.   The requirement CSIRT-IE RFC2350 provides basic information about a CSIRT   including contact details and its roles and responsibilities.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Digital Service Providers                             & Defines   responsibilities for digital service providers.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & Presents   guidelines to inform about cyber security roles and responsibilities for   operators of essential services. (Detail standards)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                 \\ \hline
\multirow{4}{*}{5}   & \multirow{4}{*}{What approaches are in place for threat   profiling and managing information security risks and vulnerabilities?}                      & Operators of   Essential Service                      & \begin{tabular}[c]{@{}l@{}}Secion   A. Identify\\      v. Risk Management Strategy\\      vi. Supply Chain Risk Management\\      Appendix B: Security Guidelines\\      Categories:\\      - Risk Management Strategy (ID.RM)\\      - Supply Chain Risk Management (ID.SC)\\      Subcategories:\\      - PR.SP-12: A vulnerability management plan is developed and implemented to   remediate vulnerabilities in a timely manner, commensurate with the risk.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             & \multirow{4}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & \begin{tabular}[c]{@{}l@{}}ISMS   Focus Area 2 – Adopt a Risk Management Approach \\      Appendix C: Information Security Frameworks \\      NIST Risk Management Framework (RMF)\\      ENISA (D1) - Governance and risk management\\      ISO 27002 (A.12.6) - Technical vulnerability management\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & \begin{tabular}[c]{@{}l@{}}STEP   4. Define your risk appetite\\      STEP 6. Implement basic protections (vulnerability management)\\      STEP 12. Create a cyber risk management lifecycle\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & The National Cyber Security Centre (NSCS)             & The   National Cyber Security Centre (NCSC) is regularly publishing Alerts \&   Advisories on cyber security issues that may affect Ireland   (https://www.ncsc.gov.ie/news/)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              &                                 \\ \hline
\multirow{3}{*}{6}   & \multirow{3}{*}{To what extent is information security   management training developed and disseminated?}                                              & National   CS Strategy                                & Skillnet   Ireland launched their Cyber Security Skills Initiative to deliver a broad   programme of initiatives in the field. Government has launched Future Jobs   Ireland, a multiannual framework for skills and enterprise development,   including the technology sector. Ireland offers a significant number of   courses in cyber security, with at least 8 Masters level courses now on   offer                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & \multirow{3}{*}{4}              \\ \cline{3-4}
                     &                                                                                                                                                        &                                                       & NATO                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & All   users are informed and trained on cyber security policies and relevant   procedures, with periodic updates. (Detail standards)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                 \\ \hline
\multirow{3}{*}{7}   & \multirow{3}{*}{To what extent is information security   management training developed and disseminated?}                                              & Incident   notification for DSPs                      & Incident   notification for DSPs in the context of the NIS Directive: As part of the EU   Cybersecurity strategy the European Commission proposed the EU Network and   Information Security directive. The NIS Directive (see EU 2016/1148) is the   first piece of EU-wide cybersecurity legislation. IS imposes security   measures and incident reporting obligations for Operators of Essential   Services (OES) and Digital Service Providers (DSP).                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & \multirow{3}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & National CS Strategy                                  & Details   implementation plan of actions relating to these measures - Information Note   for Digital Service Providers                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            &                                 \\ \hline
\multirow{3}{*}{8}   & \multirow{3}{*}{To what extent are implementation frameworks   developed and standards adopted?}                                                       & National   CS Strategy                                & Complete   first phase of Operators of Essential Services (OES) Self-Assessment against   Security Control Framework                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & \multirow{3}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & Appendix A: Framework   Infographics Appendix B: Security Guidelines                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & Appendix C:   Information Security Frameworks                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              &                                 \\ \hline
\multirow{3}{*}{9}   & \multirow{3}{*}{To   what extent are risks and challenges for cybersecurity implementation plans   identified and addressed?}                          & National   CS Strategy                                & National   Cybersecurity Strategy 2019 Cybersecurity challenges described in general                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & \multirow{3}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & Appendix   D: Sources of Information in Relation to Threats and Vulnerabilities                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & AmCham GCS Report                                     & The   American Chamber recommends addressing cyber security challenges through the   Disruptive Technologies Innovation Fund which would meet societal, in   addition to commercial, priorities and enhance Ireland’s global research   reputation Resourcing of teams and retention of talent is a challenge for An   Garda Síochána and the Defence Forces, similar to private sector experiences   in this regard.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                 \\ \hline
\multirow{5}{*}{10}  & \multirow{5}{*}{To what extent are the emerging technologies and   future trends for VTI\&CM identified?}                                              & National CS   Strategy                                & Executive   Summary (some emerging technologies listed)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \multirow{5}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & AI Cybersecurity   Challenges                         & \begin{tabular}[c]{@{}l@{}}AI   may expose individuals and organizations to new, and sometimes unpredictable,   risks, and it may open new avenues in attack methods and techniques, as well   as creating new data protection challenges, especially in safety-critical   deployments such as in autonomous vehicles, smart manufacturing, eHealth,   etc.\\      \\      In this document, Chapter 4 introduces the threat taxonomy of AI systems,   where relevant threats are presented and mapped to corresponding   assets:\\      \\      - Data\\      - Model\\      - Actors\\      - Processes\\      - Environment/Tools\\      - Artefacts\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & Other   Useful Sources                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & Background   (IoT mentioned)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & AmCham GCS Report                                     & The   main trends in the 2018 cyberthreat landscape, as identified by the European   Union Agency for Network and Information Security (ENISA) 19 showcase a range   of hot-button issues                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                 \\ \hline
\multirow{3}{*}{11}  & \multirow{3}{*}{How does the government define security   architectures guidelines  and tools for   VTI\&CM?}                                          & IS Management                                         & Suggests   strategies and activities to enhance the Information Security Posture for   improving governance around ICT in the Public Service. The security posture   is defined as the security status of an enterprise’s networks, information,   and systems based on information architecture resources (e.g. people,   hardware, software, policies) and capabilities in place to manage the defence   of the enterprise and to react as the situation changes.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & \multirow{3}{*}{2}              \\ \cline{3-4}
                     &                                                                                                                                                        & CS   Guidance for Business                            & \begin{tabular}[c]{@{}l@{}}organisations   should\\      consider additional protections to further reduce the risk of cyberattacks.   such as echnologies which support Access Management (IAM) and Vulnerability   Management (VM), and in particular the centralisation and automation of IAM   and VM processes will deliver efficiencies and cost savings. Consideration   should be given to establishing a formal role/function which considers   security architecture in all aspects of your organisation’s IT programme. It   is particularly important for organisations who develop software/systems that   security is embedded at all stages throughout the Systems Development   Lifecycle.\\      \\      Recommendation baed on NIST Special Publication 800-39 Managing Information   Security Risk.\end{tabular}                                                                                                                                                                                                                                                                                                                                        &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Digital   Service Providers                           & The systematic   management of network and information systems which means amapping of   information systems and the establishment of a set of appropriate policieson   managing information security, including risk analysis, human resources,   security ofoperations, security architecture, secure data and system   lifecycle management andwhere applicable, encryption and its management.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         &                                 \\ \hline
\multirow{5}{*}{12}  & \multirow{5}{*}{To what extent are documents to define,   implement, and monitor measures to protect IT devices established?}                          & CS Asset Management Report                            & The report   highlights that devices that are exposed to a high number of known   vulnerabilities for a lengthy period of time are more vulnerable to malicious   actors who may gain unauthorised access to IT assets and compromise the   confidentiality, integrity and availability of stored business critical data.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & \multirow{5}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & Provides   the  guidelines  and recommendations for Information   Security Management  based on standards   such as the ISO 27002 Security Control Categories and Control Objectives   which specifies the control description for mobile devices and teleworking.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & Recommends   to establish comprehensive anti-malware protection, both at the host (on   every computer,  server, mobile device,   etc.) and network-level (at email/web gateways, etc.) as a basic protection   for Irish busines. Additionally, it recommends establishing remote   access/remote working controls, including secure access to systems and   controls on the devices which may be used to access internal systems and   using full disk encryption on all mobile devices, such as laptops and   removable media (USB keys).                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & National CS Strategy                                  & The   progressive dependence of Critical National Infrastructure and services on   network-connected devices has led to the State taking a series of measures to   ensure the resilience of certain categories of critical national   infrastructure. This strategy provides a comprehensive section (6) on   Critical National Infrastructure Protection and related measures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & \begin{tabular}[c]{@{}l@{}}This   guideline presents the measures for Asset Management, including data,   personnel, devices, systems, and facilities. Please see Appendix B: Security   Guidelines for recommended practices and standards to develop and implement   the appropriate and proportionate security measures:\\      - Asset Management (ID.AM)\\      - Identity Management, Authentication and Access Control (PR.AC)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         &                                 \\ \hline
\multirow{7}{*}{13}  & \multirow{7}{*}{What information about threats is available at   the country level?}                                                                   & IS Management                                         & \begin{tabular}[c]{@{}l@{}}Appendix D   offers some potential information sources to stay abreast of the latest   threats, vulnerabilities, and potential security control options. This   includes:\\      \\      - ENISA (Annual) Threat Landscape (ETL) Report provides an overview of threats,   together with current and emerging trends.\\      \\      - ENISA Advisory Info Notes provides the information in relation to the   latest threats and vulnerabilities.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & \multirow{7}{*}{4}              \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & This   guidance provides clear steps which organisations should include to   understand who might want to attack them, why, and how they might go about   carrying out such an attack in order to allow organisations to focus the   efforts on how to respond to the most likely threats. For example, it   recommends to establish a Cyber Threat Intelligence (CTI) capability which   enables organisations to identify (through intelligence sources/feeds) and   understand the top 5-10 threat actors and likely attack scenarios (these are   your key cyber risks) and record them in a risk register. Please, see section   3. Understand the Threats.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Incident Report Form                                  & This   incident report form includes a section of lessons learned based on new   threats identified.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & National CS Strategy                                  & \begin{tabular}[c]{@{}l@{}}-   Expanding the current Threat Sharing Group (TSG) which was established in   2017. The TSG acts both as a forum for critical national infrastructure   operators, and a means for State Actors (including Gardaí and Defence Forces)   to share information with these operators and to engage with cybersecurity   professionals.\\      \\      - The NCSC has developed a threat intelligence database that is being used   to assist Agencies and Departments in protecting their networks. \\      \\      - The CSIRT has a proactive position that includes the deployment and use   of MISPs (Malware Information Sharing Platform) to share threat intelligence   directly with Critical National Infrastructure Providers, and the evolution   and use of a series of tools to identify, parse and analyse open-source   intelligence (OSINT). The CSIRT has also developed, tested, and deployed the   ‘Sensor’ platform, now operational on the infrastructure of a number of   Government Departments, to detect and warn of certain types of threat.\end{tabular}                                                              &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & The National Cyber Security Centre (NSCS)             & \begin{tabular}[c]{@{}l@{}}The   National Cyber Security Centre (NCSC) is regularly publishing Alerts \&   Advisories on cyber security issues that may affect Ireland   (https://www.ncsc.gov.ie/news/) The latest published alerts are the   following: \\      - 11-03-2021 Critical Vulnerabilities in F5 products\\      - 10-03-2021 Critical Vulnerabilities in Microsoft Exchange Servers Update   2 \\      - 25-02-2021 Unauthorised RCE in VMware vCenter \& ESXi \\      - 10-02-2021 Windows TCP/IP Remote Code Execution \& DoS Vulnerabilities\\      - 25-01-2021 SonicWall Vulnerability\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & The European Union Agency for Cybersecurity   (ENISA) & \begin{tabular}[c]{@{}l@{}}ENISA   is the Union’s agency dedicated to achieving a high common level of   cybersecurity across Europe. ENISA provides the reports EU on threats as   below:\\      - ENISA (Annual) Threat Landscape (ETL) Report provides an overview of   threats, together with current and emerging trends. For example, ENISA Threat   Landscape 2020 - List of top 15 threats.\\      \\      - ENISA Advisory Info Notes provides the information in relation to the   latest threats and vulnerabilities.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & Appendix   B outlines the best practices and informative references recommended by the   government for Operators of Essential Service in order to manage cyber threat   information.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                 \\ \hline
\multirow{4}{*}{14}  & \multirow{4}{*}{What information about threats actors is   available at the country level?}                                                            & CS Guidance for Business                              & \begin{tabular}[c]{@{}l@{}}This guidance   provides clear steps which organisations should follow to defend their   business against threat actors. Please, refer to the following   sections:\\      \\      3. Understand the threats: Threat actors (cyber criminals, malicious   insiders, etc.) vary in capability and sophistication, whilst also constantly   changing depending on the value of the prize they seek to exploit.\\      \\      5. Focus on education and awareness Establish an education and awareness   programme, ensuring all of your employees, contractors and third parties can   identify a cyberattack and are aware of the role they play in defending your   business against threat actors.\\      \\      7. Be able to detect an attack: Threat actors are many and sophisticated,   and dedicated attackers have a high chance of breaching organisations'   defences given enough time and persistence.\end{tabular}                                                                                                                                                                                                               & \multirow{4}{*}{4}              \\ \cline{3-4}
                     &                                                                                                                                                        & National CS Strategy                                  & This   document identifies key threat actors such as those state-sponsored entities,   usually military or security organisations, seeking to use network and   information systems to conduct operations ranging from the exfiltration of   data to the destruction of physical infrastructure. These threat actors,   usually referred to as ‘advanced persistent threats’ (or APTs) have been   shown to be involved in attacks across a wide range of sectors, but with a   particular focus on Government IT systems, telecommunications networks,   financial services, and technology companies.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & The National Cyber Security Centre (NSCS)             & \begin{tabular}[c]{@{}l@{}}The   National Cyber Security Centre (NCSC) is regularly publishing Alerts \&   Advisories on cyber security issues that may affect Ireland   (https://www.ncsc.gov.ie/news/) The latest published alerts are the   following: \\      - 11-03-2021 Critical Vulnerabilities in F5 products\\      - 10-03-2021 Critical Vulnerabilities in Microsoft Exchange Servers Update   2 \\      - 25-02-2021 Unauthorised RCE in VMware vCenter \& ESXi \\      - 10-02-2021 Windows TCP/IP Remote Code Execution \& DoS Vulnerabilities\\      - 25-01-2021 SonicWall Vulnerability\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & The European Union Agency for Cybersecurity (ENISA)   & \begin{tabular}[c]{@{}l@{}}ENISA   is the Union’s agency dedicated to achieving a high common level of   cybersecurity across Europe. ENISA provides the reports EU on threats as   below:\\      - ENISA (Annual) Threat Landscape (ETL) Report provides an overview of   threats, together with current and emerging trends. For example, ENISA Threat   Landscape 2020 - List of top 15 threats.\\      \\      - ENISA Advisory Info Notes provides the information in relation to the   latest threats and vulnerabilities.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              &                                 \\ \hline
\multirow{5}{*}{15}  & \multirow{5}{*}{To what extent are data security classification   guidelines established?}                                                             & CS Asset   Management Report                          & This document   outlines key findings in Irish Asset Management Firms. For example,   deficiencies in IT asset inventories were identified, where the inventories   did not capture the complete IT estate and / or classify assets (e.g., data   assets)  by their business criticality.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & \multirow{5}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & This   document recommends the ISO 27002 Security Control Categories and Control   Objectives which outlines the Information classification as part of the Asset   management.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & \begin{tabular}[c]{@{}l@{}}This   guide recommends that organisations should classify assets (e.g., data).   Please see, 2. Identify what matters most: \\      \\      Establish a comprehensive technology asset management  programme which includes all of the assets   above and ranks/classifies them by criticality to your business in a   centralised asset inventory.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Digital Service Providers                             & This   document recommends mapping secure data to appropriate policies on managing   information security. Please see 3.1 Article 16 (1).                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & This guideline   presents the measures for Asset Management, including data, personnel,   devices, systems, and facilities. Please see Appendix B: Security Guidelines   which outlines the best practices for data classification as part of the   Asset Management (ID.AM)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &                                 \\ \hline
\multirow{2}{*}{16}  & \multirow{2}{*}{To what extent is data life cycle management   addressed by the government?}                                                           & CS Guidance for   Business                            & \begin{tabular}[c]{@{}l@{}}This guide   recommends the management of data lifecysle. Please see, 6. Implement basic   protections\\      \\      Establish a data security programme, which focuses on how data is stored   and secured in organisations. This involves mapping of data locations and   flows at step two above, and then focusing on how it is protected at every   step in its lifecycle.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & \multirow{2}{*}{2}              \\ \cline{3-4}
                     &                                                                                                                                                        & Digital Service Providers                             & This   document recommends mapping information systems and the establishment of   appropriate policies on managing information security, including secure data   and system lifecycle management. Please see 3.1 Article 16 (1).                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           &                                 \\ \hline
17                   & To what extent   is data security administration addressed by the government?                                                                          & Data Protection   Regulation                          & \begin{tabular}[c]{@{}l@{}}The Data Protection Commission   (DPC) is the national independent authority responsible for upholding the   fundamental right of individuals in the EU to have their personal data   protected. The DPC is the Irish supervisory authority for the General Data   Protection Regulation (GDPR). (https://www.dataprotection.ie/)\\      \\      There is comprehensive data protection legislation (up to date as of   31.01.2019).   (https://www.dataprotection.ie/en/dpc-guidance/law/data-protection-legislation)\\      \\      There are guidelines and checklists for organizations   (https://www.dataprotection.ie/en/organisations)\\      \\      There is information on own rights for individuals   (https://www.dataprotection.ie/en/individuals,   https://www.citizensinformation.ie/en/government\_in\_ireland/national\_government/standards\_and\_accountability/data\_protection.html\#)\\      \\      There are up-to-date reports   (https://www.dataprotection.ie/en/dpc-guidance/publications)\\      \\      It is possible to report a breach or raise a complaint   (https://www.dataprotection.ie/)\end{tabular} & 3                               \\ \hline
\multirow{5}{*}{18}  & \multirow{5}{*}{To   what extent are identity and data access management addressed by the   government?}                                               & National CS   Strategy                                & Section   7.3: Measures 8. The NCSC will develop a baseline security standard to be   applied by all Government Departments and key agencies. These standards   typically include measures and controls in relation to staff training,   identity and access management.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & \multirow{5}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & Operators of Essential Service                        & Section   4 B: Protect i. Identity Management, Authentication and Access Control                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Digital Service Providers                             & Section   3.1: Article 16 (1) (d)the access controls to network and information systems   which means the availability of a set of measures to ensure that the physical   and logical access to network and information systems, including   administrative security of network and information systems, is authorized and   restricted based on business and security requirements.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & Appendix   C: Information Security Frameworks ISO 27002 (A.9) - Access Control                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & STEP   6. Implement basic protections                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                 \\ \hline
\multirow{4}{*}{19}  & \multirow{4}{*}{What   information security guidance is provided to support business continuity   planning and management?}                            & Operators   of Essential Service                      & Appendix   B: Security Guidelines Category: Service Protection Policies, Processes and   Procedures (PR.SP) Subcategory PR.SP-9: Response plans (Incident Response and   Business Continuity) and recovery plans (Incident Recovery and Disaster   Recovery) are in place and managed Subcategory PR.SP-10: Response and   recovery plans are tested                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & \multirow{4}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & Digital Service Providers                             & Section   3.1: Article 16 (1) Business continuity management referred to in point (c)   of Article 16(1) of Directive (EU)2016/1148 means the capability of an   organisation to maintain or as appropriate restore the delivery of services   at acceptable predefined levels following a disruptive incident and shall   include: (a)the establishment and the use of contingency plans based on a   business impact analysis for ensuring the continuity of the services provided   by digital service providers which shall be assessed and tested on a regular   basis for example, through exercises; (b)disaster recovery capabilities which   shall be assessed and tested on a regular basis for example, through   exercises.                                                                                                                                                                                                                                                                                                                                                                                                                                    &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & IS Management                                         & Appendix   C: Information Security Frameworks ISO 27002 (A.17) ENISA (D6)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & STEP   9. Adopt a risk-based approach to resilience                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        &                                 \\ \hline
\multirow{5}{*}{20}  & \multirow{5}{*}{To   what extent is security incidents and near incidents management addressed by   the government?}                                   & IS Management                                         & \begin{tabular}[c]{@{}l@{}}Appendix C:   Information Security Frameworks \\      ISO 27002 (A.16) - Information security incident management \\      ENISA (D5) - Incident management\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & \multirow{5}{*}{3}              \\ \cline{3-4}
                     &                                                                                                                                                        & CS Guidance for Business                              & STEP 8.  Be prepared to react (Establish a formal   cyber incident management team who have been trained in and are following a   documented plan, which is tested at least annually.)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & OES Incident Notification Form                        & Operators of   essential services have to notify the CSIRT of an incident by using the   "Operators of Essential Services: Incident Notification Form"                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & Incident Report Form                                  & Digital   service providers have to notify the CSIRT of an incident by by using the   "Digital Service Providers: Incident Notification Form"                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              &                                 \\ \cline{3-4}
                     &                                                                                                                                                        & CSIRT-IE                                              & The government   has a unit (CSIRT, CERT, CIRT, etc.) that is specialised in national-level   cyber incident detection and response. The CSIRT-IE is responsible of the   incident response for national cyber security incidents at the government and   national levels.  &                                
\\ \hline
                     &                                                                                                                                                        &                                                       &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & 3.1                             \\ \hline



\end{tabular}
\end{table}
